Single Stream Parallelization of Recurrent Neural Networks for Low Power and Fast Inference

As neural network algorithms show high performance in many applications, their efficient inference on mobile and embedded systems are of great interests. When a single stream recurrent neural network (RNN) is executed for a personal user in embedded systems, it demands a large amount of DRAM accesses because the network size is usually much bigger than the cache size and the weights of an RNN are used only once at each time step. We overcome this problem by parallelizing the algorithm and executing it multiple time steps at a time. This approach also reduces the power consumption by lowering the number of DRAM accesses. QRNN (Quasi Recurrent Neural Networks) and SRU (Simple Recurrent Unit) based recurrent neural networks are used for implementation. The experiments for SRU showed about 300% and 930% of speed-up when the numbers of multi time steps are 4 and 16, respectively, in an ARM CPU based system.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g copyright statements.

==> body-samos.tex <==
\section{Introduction}

Neural network algorithms show high performance in many machine learning tasks, such as image classification, speech recognition, and machine translation [***]. Thus, many future embedded systems, including smartphones and cars, are expected to support several neural network algorithms. A few different neural network models are used according to the characteristics of the applications. For example, convolutional neural networks are widely used for image recognition, while recurrent neural networks widely used for speech recognition and machine translation [*]. Neural network algorithms demand a very large number of arithmetic and memory access operations for real-time operations, and also require very large parameter sizes, often exceeding a few tens of megabytes (MBs). In sever based implementations, batch processing is widely used for lowering the number of DRAM accesses. Increasing the batch size lowers the number of DRAM accesses for each stream. However, batch processing can hardly be used in many embedded applications because the application is intended for a single user. One example is an on-device automatic speech recognition on a smartphone. Although, many researches are being conducted to execute neural networks algorithms efficiently using special purpose hardware, there are still DRAM access bottlenecks unless all the parameters are stored on on-chip memory. Considering the available on-chip memory size of most embedded devices, it is yet unavoidable to store the weights on DRAM. Thus, it is very needed to constrain the number of DRAM accesses for execution of a neural network algorithm. 
Recurrent neural networks are used for sequence processing, and a sequence consists of multiple, from a few to unending, time steps. Therefore, DRAM accesses can be reduced if several time steps are processed at a time. In server based batch processing, multiple streams are processed in parallel to exploit this characteristic. However, for single sequence processing needed in embedded systems, it is very difficult to parallelize the recurrent neural networks because the feedback that includes non-linear operations is usually employed.  Although signal flow graph analysis allows some partial parallelization even for the LSTM RNN, which is most widely used but very complex, the effect is limited [*]. In addition, disconnecting parallelism using data characteristics has also been attempted, but it is difficult to apply this technique to general applications [*]. Since this difficulty is due to the nature of the neural network algorithm, it is difficult to overcome this by employing very smart parallelization or special hardware design. 
In this paper, we present a single sequence parallelization of QRNN (Quasi Recurrent Neural Network) and SRU (Simple Recurrent Unit) based recurrent neural networks, and apply multi time step parallelization for efficient implementation of these algorithms on embedded systems. QRNN and SRU algorithms contain the feed-back structure, but the feedback part can be isolated and takes a small part of the total computation. This simple feed-back structure allows multi time step parallelization even for a single stream input, and enables efficient implementations reducing DRAM accesses because one weight fetch from DRAM can be used for multiple steps. QRNN and SRU algorithms are implemented on a CPU and the execution performances are compared with those of LSTM RNNs.  
This paper is organized as follows. Section 2 explains popular recurrent neural network algorithms, including LSTM RNN, QRNN, and SRU. Their performance on acoustic modeling are also given. Section 3 presents the dependency analysis of these algorithms for multi-step processing of single stream input. Implementation of QRNN and SRU using multi-step parallelization approach is explained in Section 4. Section 5 shows the implemented results. Concluding remarks follow in Section 6. 


\section{Recurrent neural networks algorithms}
A recurrent neural network (RNN) connects the units to form a feedback along a sequence, which allows it to learn dynamic temporal behavior of a time sequence. RNNs can have internal states either by feedback or by explicitly using memory cells. This makes them applicable to tasks such as connected handwriting recognition, speech recognition, language modeling, and machine translation. A most widely used LSTM RNN and recently introduced QRNN and SRU models are reviewed. 

\subsection{Application of recurrent neural networks}
RNNs are used for sequence analysis, including text processing, speech recognition, and handwriting recognition. Also, RNN is an indispensable components for sequence generation, such as text generation and foreign language translation.  Three major RNN applications are shown in Fig. \ref{fig:rnn_app}. Fig. \ref{fig:rnn_app} (a) shows the RNN acceptor that receives a sequence of input, and then generates an output at the end of the sequence. An application of the RNN acceptor is the sentiment analysis of the input text, such as movie and restaurant reviews.  Fig. \ref{fig:rnn_app} (b) shows the RNN transducer that receives the input sequence and the corresponding output is generated at each time step. The RNN transducer is used for acoustic modeling, language modeling, and so on. Fig. \ref{fig:rnn_app} (c) shows the encoder and decoder model using RNN, where the encoder compresses the input stream and passes the compressed context to the decoder at the end of the sequence. Thus, the encoder alone is similar to the RNN acceptor. The decoder receives the compressed context as the initial state, and then generates the output as the time step increases. The representative application of the encoder-decoder architecture is the language translation. The original text to translate is applied to the encoder, and the translated text is generated from the decoder. 
In many applications, bi-directional RNN models are used, where the sequence flow goes in both directions as shown in Fig. \ref{fig:rnn_app} (d). The bi-directional RNN can be constructed by combining two RNNs operating at different directions. 
%\begin{figure}
%\includegraphics[width=\linewidth]{rnn_acceptor}
%\caption{A sample black and white graphic.}
%\end{figure}

\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{rnn_acceptor}
    \caption{RNN Acceptor.}
  \end{subfigure}
  \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{rnn_transducer}
    \caption{RNN Transducer.}
  \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{rnn_encoder_decoder}
    \caption{RNN Encoder-Decoder.}
  \end{subfigure}
  \caption{Application of recurrent neural networks.}
  \label{fig:rnn_app}
\end{figure}
\subsection{LSTM RNN}


\begin{ceqn}
\begin{align}
    &\mathbf{f}_t = \sigma(\mathbf{W}_f \mathbf{x}_t + \mathbf{U}_f \mathbf{h}_t + \mathbf{b}_f), \nonumber &&\\
    &\mathbf{i}_t = \sigma(\mathbf{W}_i \mathbf{x}_t + \mathbf{U}_i \mathbf{h}_t + \mathbf{b}_i), \nonumber &&\\
    &\mathbf{o}_t = \sigma(\mathbf{W}_o \mathbf{x}_t + \mathbf{U}_o \mathbf{h}_t + \mathbf{b}_o), \nonumber &&\\
    &\mathbf{\hat{c}}_t = \tanh(\mathbf{W}_c \mathbf{x}_t + \mathbf{U}_c \mathbf{h}_t + \mathbf{b}_c),  \nonumber &&\\
    &\mathbf{c}_t = \mathbf{f}_t \odot \mathbf{c}_{t-1} + \mathbf{i}_t \odot \mathbf{\hat{c}}_t, \nonumber &&\\
    &\mathbf{h}_t = \mathbf{o}_t \odot \tanh(\mathbf{c}_{t}). 
\end{align}
\end{ceqn}


\begin{figure}
\includegraphics[width=\linewidth]{lstm}
\caption{Block diagram of LSTM}
\label{fig:lstm}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{sru}
\caption{Block diagram of SRU}
\label{fig:sru}
\end{figure}
\subsection{LSTM RNN}

\subsection{Simple Recurrent Unit and QRNN}

\begin{ceqn}
\begin{align}
    &\mathbf{\hat{x}}_t = \mathbf{W} \mathbf{x}_t , \nonumber &&\\
    &\mathbf{f}_t = \sigma(\mathbf{W}_f \mathbf{x}_t + \mathbf{b}_f), \nonumber&&\\
    &\mathbf{r}_t = \sigma(\mathbf{W}_r \mathbf{x}_t + \mathbf{b}_r), \nonumber&&\\   
    &\mathbf{c}_t = \mathbf{f}_t \odot \mathbf{c}_{t-1} + (1 - \mathbf{f}_t) \odot \mathbf{\hat{x}}_t, \nonumber&&\\
    &\mathbf{h}_t = \mathbf{r}_t \odot \tanh{(\mathbf{c}_{t})} + (1 - \mathbf{r}_t) \odot \mathbf{x}_t. 
\end{align}
\end{ceqn}

\begin{ceqn}
\begin{align}
    &\mathbf{\hat{x}}_t = \tanh(\mathbf{W}^0  \mathbf{x}_t + \mathbf{W}^1  \mathbf{x}_{t-1}) , \nonumber &&\\
    &\mathbf{f}_t = \sigma(\mathbf{W}_f^0 \mathbf{x}_t + \mathbf{W}_f^1 \mathbf{x}_{t-1}), \nonumber&&\\
    &\mathbf{o}_t = \sigma(\mathbf{W}_r^0 \mathbf{x}_t + \mathbf{W}_r^1 \mathbf{x}_{t-1}), \nonumber&&\\   
    &\mathbf{c}_t = \mathbf{f}_t \odot \mathbf{c}_{t-1} + (1 - \mathbf{f}_t) \odot \mathbf{\hat{x}}_t, \nonumber&&\\
    &\mathbf{h}_t = \mathbf{o}_t \odot \tanh{(\mathbf{c}_{t})} . 
\end{align}
\end{ceqn}

\section{Dependency Analysis for Multi Time Step Parallel Processing}
RNN computation is executed as a sequence of $\mathbf{h}_0$, $\mathbf{h}_1$, $\mathbf{h}_2$, ... and so on, where $\mathbf{h}_t$ is the output at time step t, because evaluation of $\mathbf{h}_t$ needs $\mathbf{h}_{t-1}$ as illustrated in Eq. 1. Multiple time step processing refers the computation of $\mathbf{h}_0$, $\mathbf{h}_1$, ... and $\mathbf{h}_{T-1}$, where $T$ is the block size for parallel processing. In single step processing, the weights, which is usually tens of MBs, need to be loaded at each step, and they are used only one arithmetic.  Unless the cache size is very large to accommodate all the weights, this incurs a very large number of DRAM accesses. In multi time step processing, a weight is fetched from DRAM and used for processing multiple time steps. Usually, we fetch one row of weight matrix, and use it for computing the output for multiple time steps. As a result, the number of DRAM accesses can be reduced, approximately, in inversely proportional to the number of time steps processed at a time. 

\subsection{LSTM}
As illustrated in Eq. 1, the major computation of LSTM network is due to 8 matrix-vector multiplication operations. The matrix values are weights, which are already determined through training, while the vectors are either the input $\mathbf{x}_t$ or the previous output $\mathbf{h}_{t-1}$. As for the matrix-vector multiplication with the input $\mathbf{x}_t$, there is no difficulty in multiple time step processing. But, the matrix-vector multiplication with the previous output $\mathbf{h}_{t-1}$ cannot be conducted as a multiple time step fashion because of the dependency problem. Thus, even if we precompute the matrix-vector computation with the input vector $\mathbf{x}_t$, the number of DRAM accesses can be reduced just up to a half, when compared with the single time step processing. 

\subsection{SRU}
SRU computes the output through three matrix-vector multiplication operations as shown in Eq. 2. Here we can find that the computation of the weighted input ($\mathbf{\hat{x}}_t$), forget gate $\mathbf{f}_t$, and the output gate $\mathbf{r}_t$ can be conducted using only the weight matrices and the input $\mathbf{x}_t$. There is no dependency problem. 
In SRU, there is a dependency loop propagating the memory cell value $\mathbf{c}_t$, which is however vector element wise operations, and demanding much less operations compared to matrix-vector multiplications. Also, the vector element wise operation can be conducted up to the parallelism of layer width of the RNN, which usually have the range of 128 to 1024. Thus, the computation of $\mathbf{c}_t$ can be conducted using SIMD or multi-thread operations. The computation of output $\mathbf{h}_t$ has no dependency constraints when its input $\mathbf{r}_t$ and $\mathbf{c}_t$ are all given. 

\subsection{QRNN}
AAA
\section{Experimental results}
We have measured the execution time of LSTM RNN, SRU, and QRNN models on Intel Core i7-3930K 3.2GHz CPU and Nvidia Denver2 ARMv8 64-bit 2.0GHz CPU. Small and large RNN models are used for the experiments. As for the small model, the LSTM RNN has the cell width of 350, while the SRU has the width of 512, and the number of parameters are approximately 1M.  The large model LSTM RNN has the cell width of 700, and tat of SRU RNN has the width of 1024, by which the parameter size of both models are comparable, approximately 3M. The Intel CPU has 32KB L1 data cache and instruction cache, 256KB L2 cache, and 12288KB L3 cache. The ARM CPU has 32KB L1 data cache, 48KB instruction cache, and 2048KB L2 cache.
The program was written in C++ language, and used the BLAS for optimum execution of matrix-vector and matrix-matrix multiplications. Intel Math Kernel Library (MKL) and OpenBLAS is used for Intel CPU and ARM CPU, respectively. The highest compiler optimization level, O2, is used for this experiments. 
Table \ref{tab:small_Intel} gives the execution time and the speed-up of the small model RNNs on the Intel CPU.  The LSTM with single time step and the SRU with multiple time step parallelization are shown. `SRU-n' refers to the SRU execution with n-step parallelization. The speed-up of SRU-n is measured on the basis of the SRU-1. Here, we can find almost 400\% of speed-up when 32 step parallelization is employed. A similar result can be found for the large model RNNs. Table \ref{tab:large_Intel} shows the execution time and the speed-up of large model RNNs on the CPU.   
The experimental results on ARM CPU are given on Table 3 and 4 for the small and large models, respectively. When executing the small model on the ARM CPU, the speed-up is nearly 900\% when the number of parallelization steps is 32. The speed-up of large model RNN is very impressive, more than 1,250\%. Here, we can find that the benefit of multiple time step parallelization is bigger in ARM based systems compared to Intel CPU based computer.  This is because the benefit of reduced DRAM access due to multi time step parallelization grows when the computer system has a poor memory system, such as low bandwidth DRAM and small cache size. Also, the larger RNN model shows higher speed-up compared to the small one.
\begin{table}
  \caption{Execution time (msec) of small model RNNs on the Intel CPU.}
  \label{tab:small_Intel}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    LSTM & 673.667& -\\
    SRU-1 & 475.43& 100\% \\
    SRU-2 & 288.729& 164.7\%\\    
    SRU-4 & 197.765& 240.4\%\\
    SRU-8 & 153.39& 309.9\%\\
    SRU-16 & 129.591& 366.9\%\\
    SRU-32 & 118.247& 402.1\%\\            
    SRU-64 & 96.302& 493.7\%\\            
    SRU-128 & 93.219& 510.0\%\\                        
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Execution time (msec) of large model RNNs on the Intel CPU.}
  \label{tab:large_Intel}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    LSTM & 2359.94& -\\
    SRU-1 & 1880.63& 100\% \\
    SRU-2 & 1104.22& 170.3\%\\    
    SRU-4 & 715.919& 262.6\%\\
    SRU-8 & 523.264& 359.4\%\\
    SRU-16 & 437.565& 429.7\%\\
    SRU-32 & 375.647& 500.6\%\\            
    SRU-64 & 335.64& 560.3\%\\            
    SRU-128 & 320.121& 587.4\%\\                        
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Execution time (msec) of small model RNNs on the ARM CPU.}
  \label{tab:small_ARM}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    LSTM & 1522.3& -\\
    SRU-1 & 902.736& 100\% \\
    SRU-2 & 484.474& 186.3\%\\    
    SRU-4 & 274.82& 328.5\%\\
    SRU-8 & 172.856& 522.2\%\\
    SRU-16 & 108.414& 832.6\%\\
    SRU-32 & 85.6596& 1053.8\%\\            
    SRU-64 & 96.1196& 939.1\%\\            
    SRU-128 & 93.3887& 966.6\%\\                        
  \bottomrule
\end{tabular}
\end{table} 

\begin{table}
  \caption{Execution time (msec) of large model RNNs on the ARM CPU.}
  \label{tab:large_ARM}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    LSTM & 4583.75& -\\
    SRU-1 & 3652.59& 100\% \\
    SRU-2 & 1925.07& 189.7\%\\    
    SRU-4 & 1078.03& 338.8\%\\
    SRU-8 & 634.951& 575.3\%\\
    SRU-16 & 392.163& 931.4\%\\
    SRU-32 & 288.659& 1265.4\%\\            
    SRU-64 & 275.078& 1327.8\%\\            
    SRU-128 & 275.658& 1325.0\%\\                        
  \bottomrule
\end{tabular}
\end{table} 

\begin{table}
  \caption{Execution time (msec) of small QRNNs on the Intel CPU.}
  \label{tab:small_qrnn_Intel}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    QRNN-1 & 1034.77& 100\% \\
    QRNN-2 & 558.107& 185.4\%\\    
    QRNN-4 & 376.691& 274.7\%\\
    QRNN-8 & 285.414& 362.5\%\\
    QRNN-16 & 239.941& 431.2\%\\
    QRNN-32 & 216.77& 477.3\%\\            
    QRNN-64 & 173.527& 596.3\%\\            
    QRNN-128 & 167.381& 618.2\%\\                        
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Execution time (msec) of large QRNNs on the Intel CPU.}
  \label{tab:large_qrnn_Intel}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    QRNN-1 & 3862.67& 100\% \\
    QRNN-2 & 2194.5& 176.0\%\\    
    QRNN-4 & 1413.61& 273.2\%\\
    QRNN-8 & 1020.05& 378.7\%\\
    QRNN-16 & 834.649& 462.8\%\\
    QRNN-32 & 711.423& 542.9\%\\            
    QRNN-64 & 631.667& 611.5\%\\            
    QRNN-128 & 600.772& 643.0\%\\                        
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Execution time (msec) of small QRNNs on the ARM CPU.}
  \label{tab:smal_qrnn_arm}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    QRNN-1 & 1580.58& 100\% \\
    QRNN-2 & 830.659& 190.3\%\\    
    QRNN-4 & 461.075& 342.8\%\\
    QRNN-8 & 323.815& 488.1\%\\
    QRNN-16 & 197.612& 799.8\%\\
    QRNN-32 & 143.158& 1104.9\%\\            
    QRNN-64 & 140.108& 1128.1\%\\            
    QRNN-128 & 142.536& 1108.9\%\\                        
  \bottomrule
\end{tabular}
\end{table}

\begin{table}
  \caption{Execution time (msec) of large QRNNs on the ARM CPU.}
  \label{tab:smal_qrnn_arm}
  \begin{tabular}{lll}
    \toprule
    Model&Execution Time&Speed-up\\
    \midrule
    QRNN-1 & 6467.72& 100\% \\
    QRNN-2 & 3356.7& 192.6\%\\    
    QRNN-4 & 1844.29& 350.6\%\\
    QRNN-8 & 1253.13& 516.1\%\\
    QRNN-16 & 712.439& 907.8\%\\
    QRNN-32 & 475.433& 1360.3\%\\            
    QRNN-64 & 469.515& 1377.5\%\\            
    QRNN-128 & 450.848& 1434.6\%\\                        
  \bottomrule
\end{tabular}
\end{table}

\begin{tikzpicture}
\begin{axis}[
    title={},
    xmode=log,
    log basis x=2,
    xlabel={Number of Parallelization Step},
    ylabel={Speed-up},
    xmin=1, xmax=256,
    ymin=0, ymax=15,
    xtick={1,2,4,8,16,32,64,128},
    xticklabels={1,2,4,8,16,32,64,128},
    ytick={0,1,2,4,6,8,10,12,14},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,1)(2,1.647)(4,2.404)(8,3.099)(16,3.669)(32,4.021)(64,4.937)(128,5.100)
    };
\addplot[
    color=red,
    mark=x,
    ]
    coordinates {
    (1,1)(2,1.703)(4,2.626)(8,3.594)(16,4.297)(32,5.006)(64,5.603)(128,5.874)
    };
\addplot[
    color=brown,
    mark=o,
    ]
    coordinates {
    (1,1)(2,1.863)(4,3.285)(8,5.222)(16,8.326)(32,10.538)(64,9.391)(128,9.666)
    };
\addplot[
    color=black,
    mark=triangle,
    ]
    coordinates {
    (1,1)(2,1.897)(4,3.388)(8,5.753)(16,9.314)(32,12.654)(64,13.278)(128,13.250)
    };
    \legend{{Small SRU, Intel CPU}, {Large SRU, Intel CPU}, {Small SRU, ARM CPU}, {Large SRU, ARM CPU}}
\end{axis}
\end{tikzpicture}


\begin{tikzpicture}
\begin{axis}[
    title={},
    xmode=log,
    log basis x=2,
    xlabel={Number of Parallelization Step},
    ylabel={Speed-up},
    xmin=1, xmax=256,
    ymin=0, ymax=15,
    xtick={1,2,4,8,16,32,64,128},
    xticklabels={1,2,4,8,16,32,64,128},
    ytick={0,1,2,4,6,8,10,12,14},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,1)(2,1.854)(4,2.747)(8,3.625)(16,4.312)(32,4.773)(64,5.963)(128,6.182)
    };
\addplot[
    color=red,
    mark=x,
    ]
    coordinates {
    (1,1)(2,1.760)(4,2.732)(8,3.787)(16,4.628)(32,5.429)(64,6.115)(128,6.430)
    };
\addplot[
    color=brown,
    mark=o,
    ]
    coordinates {
    (1,1)(2,1.903)(4,3.428)(8,4.881)(16,7.998)(32,11.049)(64,11.281)(128,11.089)
    };
\addplot[
    color=black,
    mark=triangle,
    ]
    coordinates {
    (1,1)(2,1.926)(4,3.506)(8,5.161)(16,9.078)(32,13.603)(64,13.775)(128,14.346)
    };
    \legend{{Small QRNN, Intel CPU}, {Large QRNN, Intel CPU}, {Small QRNN, ARM CPU}, {Large QRNN, ARM CPU}}
\end{axis}
\end{tikzpicture}

\section{Concluding Remarks}
RNN execution demands a large memory bandwidth, especially when only a single stream input data is processed. We have reduced the number of DRAM accesses by parallelizing the RNNs in the time domain. In this approach, one weight fetch is used for execution in multiple time steps, thus the efficiency increases as the number of time steps to parallelize grows. This parallelization technique is applied to simple recurrent units (SRUs) and quasi-RNNs (QRNNs), which are both recently developed models with a simple recurrence structure. The experiments were conducted on Intel CPU and ARM CPU based systems.  We achieved a speed-up of more than 400\% at the Intel CPU based system, and that of more than 1,250\% at the ARM CPU based system. 



\subsection{References}

\begin{acks}
  The authors would like to thank Dr. Yuhua Li for providing the
  MATLAB code of the \textit{BEPS} method.

  The authors would also like to thank the anonymous referees for
  their valuable comments and helpful suggestions. The work is
  supported by the \grantsponsor{GS501100001809}{National Natural
    Science Foundation of
    China}{http://dx.doi.org/10.13039/501100001809} under Grant
  No.:~\grantnum{GS501100001809}{61273304}
  and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
    Scientists' Support Program}.

\end{acks}

